A Step Closer to Comprehensive Answers: Constrained Multi-Stage Question Decomposition with Large Language Models

While large language models exhibit remarkable performance in the Question Answering task, they are susceptible to hallucinations. Challenges arise when these models grapple with understanding multi-hop relations in complex questions or lack the necessary knowledge for a comprehensive response. To address this issue, we introduce the "Decompose-and-Query" framework (D&Q). This framework guides the model to think and utilize external knowledge similar to ReAct, while also restricting its thinking to reliable information, effectively mitigating the risk of hallucinations. Experiments confirm the effectiveness of D&Q: On our ChitChatQA dataset, D&Q does not lose to ChatGPT in 67% of cases; on the HotPotQA question-only setting, D&Q achieved an F1 score of 59.6%. Our code is available at https://github.com/alkaidpku/DQ-ToolQA.

==> sections/draft.tex <==
外部调用工具的论文：

key idea：
问答库、问题限制、可回溯、训练自适应

Large language models (LLMs) have greatly promoted the development of natural language processing (NLP). Instruction-tuned models exhibit versatility in accommodating a wide array of instructions and find applicability across various task scenarios \citep{chung_scaling_2022, gunasekar_textbooks_2023, xu_wizardlm_2023}.
